Graph Feature Gating Networks

Graph neural networks (GNNs) have received tremendous attention due to their power in learning effective representations for graphs. Most GNNs follow a message-passing scheme where the node representations are updated by aggregating and transforming the information from the neighborhood. Meanwhile, they adopt the same strategy in aggregating the information from different feature dimensions. However, suggested by social dimension theory and spectral embedding, there are potential benefits to treat the dimensions differently during the aggregation process. In this work, we investigate to enable heterogeneous contributions of feature dimensions in GNNs. In particular, we propose a general graph feature gating network (GFGN) based on the graph signal denoising problem and then correspondingly introduce three graph filters under GFGN to allow different levels of contributions from feature dimensions. Extensive experiments on various real-world datasets demonstrate the effectiveness and robustness of the proposed frameworks.

==> acm/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acm/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations
	       

==> sections/experiment_old.tex <==
\section{Experiment}
In this section, we evaluate the effectiveness of our proposed model under different settings. In particular, we aim to answer the following research questions:
\begin{itemize}
    \item How does GFGN perform on various benchmark datasets compared with other GNN models?
    \item Does the framework work as designed? 
    \item  Can GFGN boost model robustness under severe random noise? 
\end{itemize}

\subsection{Experimental Setup}
\subsubsection{Datasets.} We conduct experiments on 9 benchmark datasets from various domains including citation, social, webpage, and actor co-occurrence networks. Specifically, we use 2 social networks including BlogCatalog and Flickr~\cite{huang2017label}, 3 webpage datasets including Texas, Cornell and Wisconsin~\cite{pei2020geom}, 1 actor co-occurrence network Actor~\cite{pei2020geom} and 3 citation graphs including Cora, Citeseer and Pubmed~\cite{kipf2016semi}. Note that BlogCatalog, Flickr, Texas, Cornell, Wisconsin and Actor are disassortative graphs where the node homophily is low (smaller than $0.5$), while the other three datasets are assoratative graphs~\cite{pei2020geom,zhu2020generalizing}.  The statistics of these datasets are shown in Table~\ref{tab:dataset}. It is also worth noting that the node attributes of BlogCatalog and Flickr are tags of user interest while the node attributes in other datasets are text descriptions (bag-of-words features).

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\caption{Dataset Statistics.}
\begin{tabular}{@{}lcccc@{}}
\toprule
Datasets    & \#Nodes & \#Edges & \#Features & \#Classes \\
\midrule
BlogCatalog & 5196    & 171743  & 8189       & 6         \\
Flickr      & 7575    & 239738  & 12047      & 9         \\
Actor       & 7600    & 33544   & 931        & 5         \\
Cornell     & 183     & 295     & 1703       & 5         \\
Texas       & 183     & 309     & 1703       & 5         \\
Wisconsin   & 251     & 499     & 1703       & 5         \\
Cora        & 2708    & 5429    & 1433       & 7         \\
Citeseer    & 3327    & 4732    & 3703       & 6         \\
Pubmed      & 19717   & 44338   & 500        & 3    \\    
\bottomrule
\end{tabular}
\label{tab:dataset}
\end{table}

\subsubsection{Baselines.}
\jw{maybe we can further elaborate on those methods.} To validate our proposed method, we compare it with representative GNN mdoels including GCN~\cite{kipf2016semi}, GAT~\cite{gat}, SGC~\cite{wu2019simplifying}, ARMA~\cite{bianchi2019graph-arma},  APPNP~\cite{klicpera2018predict-appnp} and Geom-GCN~\cite{pei2020geom}. We implemented our proposed method and most necessary baselines using Pytorch Geometric~\cite{fey2019fast-pyg}, a library for geometric deep learning extension library built upon Pytorch~\cite{paszke2017automatic-pytorch}.
 
\input{tables/node_classification}
\subsubsection{Parameter Setting.}
\label{sec:setup}
For a fair comparison, all methods are evaluated on the same data splits. We set training epochs to 1000, early stopping to 100, number of total hidden units to 64 and tune hyperparameters individually for all methods on each dataset based on the validation set. 
% With the graph filters introduced in Section~\ref{sec:framework}, we develop three model variants called GFGN-graph, GFGN-neighbor and GFGN-pair corresponding to graph-level, neighborhood-level and pair-level smoothing, respectively. 
For the three variants of GFGN, we fix the number of layers to 2, the number of heads to 8, the number of hidden units in each head to 8; we search learning rate from $\{0.005, 0.05\}$, dropout rate from $\{0.5, 0.8\}$, $\lambda$ from $\{0.5, 1, 2\}$ and $L_2$ normalization from $\{$5$e$-4, 5$e$-5$\}$.

Following the experimental setting of Geom-GCN~\cite{pei2020geom}, for all datasets except BlogCatalog and Flickr, we use 10 random splits provided by~\cite{pei2020geom}, which chooses 48\% of the nodes for training, 32\% validation and 20\% for test\footnote{Although \cite{pei2020geom} claims that the ratios are 60\%/20\%/20\%, the actual ratios of data splits provided on GitHub are 48\%/32\%/20\%.}. For BlogCatalog and Flickr, since the splits are not provided we adopt the same training/validation/test ratios  to divide the datasets. For each random split, the experiments are repeated 10 times with different random seeds. 





% \subsection{Evaluation on Synthetic Datasets}
% We can create datasets where $k$ feature channels share different homophily. Then we can vary $k$ and report the performance.


\subsection{Node Classification Performance}
\label{sec:node_classification}
% One synthetic setting could be using spectral embedding to get node features and based on these initial node features to perform the following aggregation and transformation. This setting can ensure these features have different smoothness over the graph.Also for all datasets, you can check the smoothness for each dimension. For spectural embedding, choose these dimensions with very different smoothness it eigenvalues.
To answer the first research question, we conduct node classification with comparison to existing state-of-the-art graph neural network models. We report the mean accuracy on 10 random splits for the nine datasets as well as the average rank of each algorithm in Table~\ref{tab:node_classification}. From the table, we make the following observations:
\begin{itemize}
    \item The proposed three smoothing methods consistently achieve strong performance on the 9 datasets: GFGN-graph, GFGN-neighbor and GFGN-pair achieve average ranks of $2.8$, $2.6$ and $2.7$, respectively, followed by Geom-GCN with an average rank of $4.6$. Further, among all the 9 datasets, the proposed methods achieve the best performance on 7 datasets. It is worth noting that our models bring significant improvement over GCN. For example, on Flickr and Cornell datasets, our model outperforms GCN by a margin of $25.24\%$ and $24.35\%$, respectively. The superiority of the proposed methods demonstrates the importance of treating each feature channel differently during the aggregation process of graph neural networks.
    \item Our models can bring much more significant improvement on disassortative graphs than assoratative graphs. In disassorative graphs the features between connected nodes are not as similar as those in assoratative graphs, so the methods (GCN, GAT and SGC) based on local aggregation will aggregate noisy information from neighbors, thus resulting in bad-quality node embeddings. On the contrary, as described in Section~\ref{sec:framework}, our models can learn different smoothness scores for different feature channels, which enables them to adaptively balance the information from the node itself and its neighbors. Specifically, for two connected nodes, if most of their features are dissimilar, our methods can learn to capture such information and assign small smoothness scores for those feature channels. For the detailed analysis of the learned smoothness scores, we will further investigate them in Section~\ref{sec:score_analysis}. Although our model does not improve GCN on assortative graphs as significantly as on disassortative graphs, the results show that the proposed aggregation scheme does not hurt the performance and is comparable with other SOTA graph neural network designs.
    \item Different datasets could need smoothing strategy of different granularity. For example, GFGN-graph significantly outperforms the other two GFGN variants on Wisconsin dataset, indicating that graph-level smoothing is good enough for improving the performance on this dataset while the other two might not be well trained since they need to learn more coefficients. In contrast, GFGN-pair outperforms the other two on Flickr dataset, suggesting that the finest smoothing granularity works the best on this dataset.
    % \item  The average ranks of the three variants of GFGN show that GFGN-neighbor and GFGN-pair perform better than GFGN-graph. It is because they are more flexible since they can give adaptive smoothing scores for different nodes or pairs. Further, GFGN-neighbor gets the highest rank indicating it could be the most stable model variant. We'll further verify this claim in Section~\ref{sec:params} as well as analyzing the difference among the three methods. 
\end{itemize}


\begin{figure*}[ht]%
\vskip -0.2em
    \centering
    \subfloat[BlogCatalog]
        {{\includegraphics[width=0.25\linewidth]{images/scores/BlogCatalog.pdf}}}%
    \subfloat[Flickr]{{\includegraphics[width=0.25\linewidth]{images/scores/flickr.pdf} }}%
    \subfloat[Texas]{{\includegraphics[width=0.25\linewidth]{images/scores/texas.pdf} }}%
    % \subfloat[Wisconsin]
    %     {{\includegraphics[width=0.25\linewidth]{images/scores/wisconsin.pdf}}}%
    % \qquad
    % \subfloat[Cornell]{{\includegraphics[width=0.25\linewidth]{images/scores/cornell.pdf}}}%
    \subfloat[Cora]{{\includegraphics[width=0.25\linewidth]{images/scores/cora.pdf} }}%
    % \subfloat[Citeseer]{{\includegraphics[width=0.25\linewidth]{images/scores/citeseer.pdf}}}%
    % \subfloat[Pubmed]{{\includegraphics[width=0.25\linewidth]{images/scores/pubmed.pdf} }}%
    \qquad
    % \vskip -1.2em
    \caption{The values of learned smoothing scores in the first layer of GFGN-graph.}%
    \label{fig:scores}
    \vskip -1em
\end{figure*}

\begin{figure*}[ht]%
\vskip -0.2em
    \centering
    \subfloat[BlogCatalog]
        {{\includegraphics[width=0.25\linewidth]{images/scores-2/BlogCatalog.pdf}}}%
    \subfloat[Flickr]{{\includegraphics[width=0.25\linewidth]{images/scores-2/flickr.pdf} }}%
    \subfloat[Texas]{{\includegraphics[width=0.25\linewidth]{images/scores-2/texas.pdf} }}%
    \subfloat[Cora]
        {{\includegraphics[width=0.25\linewidth]{images/scores-2/cora.pdf}}}%
    \qquad
    % \vskip -1.2em
    \caption{The values of learned smoothing scores in the first layer of GFGN-neighbor.}%
    \label{fig:scores_neighbor}
    \vskip -1em
\end{figure*}
\begin{figure*}[ht]%
\vskip -0.2em
    \centering
    \subfloat[BlogCatalog]
        {{\includegraphics[width=0.25\linewidth]{images/scores-3/BlogCatalog.pdf}}}%
    \subfloat[Flickr]{{\includegraphics[width=0.25\linewidth]{images/scores-3/flickr.pdf} }}%
    \subfloat[Texas]{{\includegraphics[width=0.25\linewidth]{images/scores-3/texas.pdf} }}%
    \subfloat[Cora]
        {{\includegraphics[width=0.25\linewidth]{images/scores-3/cora.pdf}}}%
    \qquad
    % \vskip -1.2em
    \caption{The values of learned smoothing scores in the first layer of GFGN-pair.}%
    \label{fig:scores_pair}
    \vskip -1em
\end{figure*}


\subsection{Analysis of Smoothing Scores}
\label{sec:score_analysis}
In the previous subsection, we have demonstrated the effectiveness of the proposed framework. In this subsection, we aim to perform analysis on the learned smoothing scores and answer the second research question. We first start from studying the smoothing scores in graph-level smoothing.  Specifically, we choose the scores from the first layer of GFGN-graph and plot the values with respect to different feature channels in Figure~\ref{fig:scores} for all datasets. From the results, we can make the following observations:
\begin{itemize}
    \item The learned smoothing scores in all datasets vary in some range, indicating that our model can learn different scores for different feature channels. Given the superior performance of GFGN described in Section~\ref{sec:node_classification}, treating feature channels differently and assigning different smoothing scores is of great significance to improve the performance.
    \item The variance of the scores is different across datasets. In particular, the learned scores in BlogCatalog and Flickr datasets have a much larger variance than others: the scores in BlogCatalog, Flickr and Texas vary in the range of $[0.06, 1.66]$, $[0.14,1.27]$ and $[0.04, 1.77]$, respectively, while in other datasets like Cora the range is only $[0.55, 0.87]$. It is because all the three datasets are disassortative graphs where node homophily is low. 
    
    % both of them are social networks with tags of user interests as node attributes and such features are supposed to be considered differently during aggregation; this is in line with our initial motivation that people are connected due to diverse reasons (e.g., sharing different interests with different friends) and the different interest information should contribute differently during the aggregation process. On the contrary, the node features in other datasets are text descriptions represented as bag-of-words where each feature dimension is not as meaningful as user interest. So the variance in those datasets tends to be much smaller.
    \item For those dataset with bag-of-words features, we find that the learned smoothing scores in disassortative graphs are much smaller, ranging from $[0.10, 0.25]$ while the scores in assorative graphs vary around $0.7$. This phenomenon indicates that feature information in those disassortative graphs are more important than structural information such that we should give low smoothing  scores in almost all the feature channels and aggregate less information from neighbors. 
\end{itemize}
Next we study the smoothing scores for neighborhood-level and pair-level smoothing. For neighborhood-level smoothing, we choose the scores from the first layer of GFGN-neighbor and for each channel we group the values from the same neighbor and plot them in the form of box plot in Figure~\ref{fig:scores_neighbor}. Similarly, we plot the pairwise values of scores from the first layer of GFGN-pair on each channel in Figure~\ref{fig:scores_pair}. We only show the results on BlogCatalog, Flickr, Texas and Cora since similar patterns are exhibited in other datasets. From the results, we find that both GFGN-neighbor and GFGN-pair can learn adaptive smoothing scores with respect to nodes or pairs, as well as feature channels. We also note that
the variance of the scores in each channel, represented by the height of the box, shows different trends on different datasets: on datasets with user interests as node features, i.e., BlogCatalog and Flickr, the variance is smaller than that on datasets with bag-of-words features, i.e., Texas and Cora. This suggests that \jw{don't know what we can conclude here.....}
% and more results can be found in the appendix. 

% \subsection{How does it work}
% The main goal is to verify our claim: visualize the coefficients. 

% Our model is expected to work on datasets that features not homophily and features    

\subsection{Robustness under Random Noise}
When the graph structure is injected with random noise, a lot of new connections will be created. 
%Among those connections, some connect nodes with totally different features, some connect nodes with partially similar features while some connect nodes with highly similar features. 
Considering the huge amount of the possible node pairs in the graph, most of the random connections will connect nodes with totally different features, some connect nodes with partially similar features. 
The connections that connect totally/partially dissimilar nodes will inevitably bring noisy information when traditional GNN models aggregate information from neighbors and lead to terrible performance. In contrast, our proposed GFGN can learn to balance the information from neighbors and the node itself as well as balancing the information from different feature channels, thus boosting model robustness under random noise. Specifically, for the connections that connect partially dissimilar nodes, GFGN is expected to learn low smoothing scores for those dissimilar feature channels while learning high smoothing scores for those similar channels.

In this subsection, we aim to evaluate how our model behaves under different severity of random noises. Specifically, we conduct the experiments on Cora, Citeseer and Pubmed datasets. Specifically, we inject random noise into the graph structure by randomly adding a certain ratio of edges. We vary the ratio from 0\% to 100\% with a step size of 20\%. To conduct experiments, we follow the same experimental setting, i.e. random splits and hyper-parameter search space, as described in Section~\ref{sec:setup}
and report the node classification accuracy in Figure~\ref{fig:robustness}. The figure shows that the proposed three mechanisms can consistently outperform all other baselines and our methods are more robust under random noise. As we can see from the figure, GFGN consistently outperforms other baselines under different severity of random noise on all the three datasets. Specifically, under $100\%$ random noise, GFGN improves GCN by a margin of $3.5\%$, $4.8\%$ and $8.1\%$ on Cora, Citeseer, Pubmed, respectively. It demonstrates that the proposed GFGN is more robust under random noise than traditional graph neural network models.

\begin{figure*}[tb]%
%\vskip -0.2em
     \centering
     \subfloat[Cora]{{\includegraphics[width=0.33\linewidth]{images/cora.pdf} }}%
     \subfloat[Citeseer]{{\includegraphics[width=0.33\linewidth]{images/citeseer.pdf} }}%
    \subfloat[Pubmed]{{\includegraphics[width=0.33\linewidth]{images/pubmed.pdf} }}%
    \qquad
    \vskip -0.25em
    \caption{Node classification accuracy under different ratio of random noise.}
    \label{fig:robustness}
\vskip -0.25em
\end{figure*}

% \subsubsection{Structural noise}

% \subsubsection{Feature noise}
% Performs even worse. Although we have the feature importance vector, it is applied on the features that has been transformed so it is hard to say that it can really denoise the noised original feature. 

% For noisy features, it should give higher smoothness coefficients to denoise; for noisy structure, it should give lower smoothness coefficients to denoise.

\begin{figure}[tb]%
\vskip -1em
    \centering
    \subfloat[BlogCatalog]{{\includegraphics[width=0.5\linewidth]{images/params/blogcatalog.pdf} }}%
    \subfloat[Cornell]{{\includegraphics[width=0.5\linewidth]{images/params/cornell.pdf} }}% 
    \quad
    \subfloat[Cora]{{\includegraphics[width=0.5\linewidth]{images/params/cora.pdf} }}%
    \subfloat[Pubmed]{{\includegraphics[width=0.5\linewidth]{images/params/pubmed.pdf} }}%
    \vskip -1em
    \caption{Results of parameter analysis on four datasets.}%
    \label{fig:params}%
\vskip -1em
\end{figure}

\subsection{Parameter Analysis}
\label{sec:params}
In this subsection, we  explore how the value of  hyper-parameter $\lambda$ impacts the performance of the three variants of GFGN. We vary the value of $\lambda$ and only report the results on BlogCatalog, Wisconsine, Cora and Pubmed since similar observations are made in other datasets. Note that when $\lambda=0$, GFGN reduces to multilayer perceptron (MLP). The performance change of GFGN is shown in Figure~\ref{fig:params} and we make the following observations:  

\begin{itemize}
    \item When choosing an appropriate value of $\lambda$, GFGN consistently outperforms MLP which does not incorporate the graph structural information. However, a large value of $\lambda$ can hurt the performance. This could be the reason that large $\lambda$ allows too much freedom in learning the smoothing scores and makes the training process unstable.  
    \item Among the three variants of GFGN, GFGN-neighbor tend to be more stable than the other two. Specifially, when the value of $\lambda$ increases, GFGN-graph is very sensitive and the performance drops rapdily; GFGN-pair also suffers the same issue. GFGN-graph assigns the same smoothing score vector for all nodes, which is not flexible for the individuals; GFGN-pair requires to learn a score for each node pair and it becomes harder to learn good scores for each when the graph is dense (like BlogCatalog). Compared with them, GFGN-neighbor can learn adaptive scores for each node and the number of scores vectors is not too many to learn. Hence, in practice, we suggest to use GFGN-neighbor first before trying the other two variants.
    %\item Disassortative graph with bag-of-words features (Wisconsin) favors small value of $\lambda$ while assorative graphs favors larger value of $\lambda$. Since $\lambda$ controls the range of output of the gates, it directly affects the smoothing scores. Disassortative graph would favor small smoothness while assortative graph would favor large smoothness. Hence, if we have some prior knowledge (e.g., estimated homophily) on the graph data, we can set it to a proper value to help train the proposed method.  
\end{itemize}


==> sections/intro_old.tex <==
\section{introduction}
\jt{I will rewrite the whole introduction. You can keep this version. I want to use this as an example to show to our group to how to write an introduction. Wei, you can move to other sections and do not need to make any changes to it from now.}

Many types of real-world data can be naturally represented as graphs. For example, social and biological networks... application

A standard approach to the analysis of sparse graphs consists in embedding the graph in some vector space of low dimension. Spectral embedding selects top k eigenvectors as the embeddings of nodes and each node corresponds to xxx. Eigenvalues indicate the smoothness of the eigenvectors~\cite{...}. Specifically, the eigenvector corresponding to small eigenvalue varies slowly across the graph, i.e., the values of the eigenvector at two connceted nodes are likely to be similar. In this sense, each channel of the embedding has different smoothness. Spectral embedding has been demonstrated to be successful in many applications, such as ...~\cite{..}. However, it only exploits the information of graph structure and lacks the capability of leveraging node features, which makes it not applicable on attributed graphs. 

Another approach for generating node embeddings falls into graph neural networks, which can capture both structure and feature information simultaneously. \jw{GNN message passing...} However, current GNNs do not specify different smoothness for different feature channels and they may fail to evaluate the contribution from the neighbors fairly. Allowing different feature channel to contribute differently is important for generating node embeddings since in real-world scenarios the smoothness of different feature channels varies. For example, in a social network, user attributes often consist of gender, marital status, interest, location, etc. Two connected users are expected to share similar interest and close location while their gender and marital status could be quite different. \jw{we can include a figure to illustrate it.}In such graphs, some feature channels follow the homophily assumption well while others may not. \tyler{although never mentioned in these GNN papers it is also due to social influence and not just social homophily, since homophily suggests users will connect to users having similar features, but influence suggests once users are connected their features become similar and are smoothed.. probably not include, but just wanted to comment} Hence, when generating node embeddings for such networks, we should allow different features to contribute differently during the aggregation process. It is worth noting that although the graph attention network (GAT) can learn attention scores to measure the contribution of neighbors, it still treats each feature channel equally. Then a natural question is how to enable current GNNs with the capability of assigning different smoothness levels to different feature channels. % We can also motivate our proposed method from the message-passing mechanism of GNNs. 

In this paper, we start from the basic graph signal denoising problem and extend it to three graph filters with different smoothing granularity levels.


% \jw{interpretable?} 

% Motivation: 
% For disassorative graphs, some feature dimension are not smooth (not homophily), we can choose not to aggregate them.


==> sections/intro_www.tex <==
\section{Introduction}
Many types of real-world data can be naturally denoted as graphs such as social networks, transportation networks, and biological networks~\cite{battaglia2018relational-survey,wu2019comprehensive-survey,zhou2018graph-survey}.  Recent years have witnessed great success from graph neural networks (GNNs) in extracting effective graph representations and tackling graph-related applications~\cite{wu2019comprehensive-survey,zhou2018graph-survey}. GNNs adopt a message-passing scheme, where for each given node, its node representation is obtained by aggregating and transforming the representations of its neighbors~\cite{mpnn}.
Specifically, in most graph neural network layers, node $v_i$'s representation is updated through the following process,
% \jt{here you can focus on the aggregation process of GCN and write its formulation for a node $v_i$, I think it is clearer to show that it gives equal importance to each feature dimension. }
% \begin{equation}
% \mathbf{H}_{i} \leftarrow  \operatorname{Transform}\left(  \operatorname{Aggregate}\left(\{\mathbf{H}_{i}, \{\mathbf{H}_{j} \mid j \in \mathcal{N}(v_i)\}\}\right) \right),
% \end{equation}
% Specifically, in a single graph neural network layer, the aggregation process for node $v_i$ can be formulated as follows,
% \begin{align}
% & \mathbf{M}_i =  \operatorname{Aggregate}\left(\mathbf{H}_{j} \mid j \in \mathcal{N}(v_i)\right)
% \end{align}
\begin{align}
\mathbf{H}_{i} \leftarrow \operatorname{Transform}(\sum\limits_{j\in \mathcal{N}(v_i)\cup{\{v_i\}}} c_{ij}{\bf H}_j), 
\label{eq:GNNaggregation}
\end{align}
 where ${\bf H}_i\in \mathbb{R}^{1\times d}$ is the representation of node $v_i$ with $d$ indicating its dimension, $\mathcal{N}(v_i)$ denotes the neighborhood of $v_i$, and $c_{ij}$ is the aggregation coefficient for the node pair $(v_i, v_j)$. Though the existing GNNs consider different contributions of neighbors via $c_{ij}$, they use the exact same strategy (coefficients) to aggregate information from each feature dimension (or each dimension of ${\bf H}_j$). This naturally raises the question: should we consider each feature dimension differently during the aggregation?

{\bf Motivation Example 1: Spectral Embedding.} By selecting top eigenvectors of the graph Laplacian matrix as the node representation, the method of spectral embedding embeds the graph into a low-dimensional space where each dimension corresponds to an eigenvector~\cite{von2007tutorial,ng2002spectral}.
Specifically, given the adjacency matrix $\mathbf{A}$ with $\mathbf{D}$ as its degree matrix, its $k$-th eigenvector $\mathbf{f}_k$ can be obtained through $({\bf D} - \mathbf{A}){\mathbf f}_k = \lambda_k \mathbf{f}_k$ with $\lambda_k$ as the $k$-th eigenvalue. In fact, $\mathbf{f}_k$ denotes the $k$-th dimension of node representations (or the vector with the $k$-th feature of all nodes)~\footnote{In practice, $\mathbf{f}_k$ is the $k-1$ dimension of node representations since we often eliminate the first eigenvector that has the same value for all nodes}. Focusing on the $i$-th element of $\mathbf{f}_k$ (or the node $v_i$), denoted as $\mathbf{f}_k(v_i)$, we have: 
\begin{align}
& d_{v_i}\mathbf{f}_k(v_i) -\sum\limits_{j\in \mathcal{N}(v_i)} {\bf f}_k({v_j}) = \lambda_k \mathbf{f}_k(v_i) \nonumber \\
\Rightarrow \quad  & \mathbf{f}_k(v_i) = \frac{1}{d_{v_i}-\lambda_k} \sum\limits_{j\in \mathcal{N}(v_i)} {\bf f}_k({v_j}), 
\label{eq:spectral_embed}
\end{align}
where $d_{v_i}$ is the degree of $v_i$. Eq.~\eqref{eq:spectral_embed} indicates the aggregation process of the $k$-th feature dimension of $v_i$ from $v_i$'s neighbors. The process uses the coefficient $\frac{1}{d_{v_i}-\lambda_k}$ for the $k$-th dimension. Since $\lambda_k$ is different for each dimension, Eq.~\eqref{eq:spectral_embed} suggests that spectral embedding treats each feature dimension differently which is controlled by $\lambda_k$. From $({\bf D} - \mathbf{A}){\mathbf f}_k = \lambda_k \mathbf{f}_k$, we have $\mathbf{f}_k^T({\bf D} - \mathbf{A}){\mathbf f}_k = \lambda_k \|\mathbf{f}_k\|^2 = \lambda_k$ if $\|\mathbf{f}_k\|^2 = 1$. Thus, $\lambda_k$ measures the smoothness of the feature dimension $\mathbf{f}_k$ over the graph. 
% the eigenvector corresponding to small eigenvalue varies slowly across the graph, i.e., the values of the eigenvector at two connceted nodes are likely to be similar. In this sense, each channel of the embedding has different smoothness. Spectral embedding has been demonstrated to be successful in many applications, such as ...~\cite{..}. However, it only exploits the information of graph structure and lacks the capability of leveraging node features, which makes it not applicable on attributed graphs. 



\begin{figure}[tb]%
%\vskip -0.2em
     \centering
     \subfloat[Dimension 1]{{\includegraphics[width=0.5\linewidth]{images/dimension1.pdf} }}%
     \subfloat[Dimension 2]{{\includegraphics[width=0.5\linewidth]{images/dimension2.pdf} }}%
    \qquad
    \label{fig:robustness}
\end{figure}

\wei{mtrust figures}
 {\bf Motivation Example 2: Social Dimension Theory.} Social dimension theory indicates that the connections in social media are not homogeneous since different people are connected due to diverse reasons~\cite{tang2009relational,tang2009scalable}. To better illustrate this theory, we show a toy example in Figure~\ref{fig:toy}. Each user is associated with an attribute vector where the elements indicate user's interests in books, movies and sports, respectively. User 1 connects to User 2 because they both subscribe the topics related to books and movies so the first two elements of their attribute vector is $1$ while User 1 connects to User 3 because they often watch similar sport games so the third element of their attribute vectors is $1$. From the toy example, social dimension theory suggests that users are often similar in only some aspects (or some attribute dimensions). In addition to social graphs, social dimension theory can be applied to other types of graphs. For example, in a website graph, a website can connect to other websites (e.g., advertisement websites and donation websites) for different reasons (or different feature dimensions). %Hence, it is of great significance to enable current GNNs with the capability of dealing with such heterogeneous relations. Since the types of the relations are often unknown or latent, we can focus on feature-level to address the aforementioned issue, i.e., allow different feature channels to contribute differently during the aggregation process. 

The aforementioned two motivation examples suggest that we should consider each feature dimension differently during the aggregation process. Thus, in this paper, we aim to design a new aggregation scheme which enables feature dimensions to contribute  differently to the aggregation process. Inspired by the general framework recently introduced in~\cite{ma2020unified}, we introduce a general graph feature gating network (GFGN) based on the graph signal denosing problem. Based on GFGN, we introduce three graph filters that allow different-level contributions of feature dimensions. Our contributions can be summarized as follows:
\begin{itemize}
    \item Based on the graph signal denoising problem, we design a general framework GFGN that allows different feature dimensions to contribute differently during aggregation.
    \item Under the general framework of GFGN, we propose three graph filters to capture different-level contributions of feature dimensions.
    \item Extensive experiments on various datasets validate the effectiveness and advantages of the proposed GFGN. We also demonstrate that GFGN is more robust to random noise.
\end{itemize}
% In essence, we mainly address two challenges: (1) how to design an aggregation that allows different feature dimensions to contribute differently? (2) how to understand the new design?  To address the first challenge, we propose a feature gating mechanism which learns a gating score for each feature channel. Inspired by the general framework recently introduced in~\cite{ma2020unified}, for the second challenge, we connect the new aggregation scheme with the graph signal denoising problem.  This connection not only provides a deep understanding on the design but also enables us to develop new aggregations. Our contributions can be summarized as follows:
% \begin{itemize}
%     \item We design a new aggregation scheme for GNNs with feature gating mechanism that allows different feature dimensions to contribute differently during aggregation.
%     \item Under the new aggregation scheme, we propose three graph filters to capture different levels of contributions of feature dimensions  from the perspective of the signal denoising problem.
%     \item Extensive experiments show that the proposed GFGN is able to achieve the state-of-the-art performance on various datasets. We also demonstrate that it is more robust than other GNN methods with the present of severe random noise.
% \end{itemize}


%In such graphs, some feature channels follow the homophily assumption well while others may not. Hence,  when generating node embeddings for such networks, we should allow different features to contribute differently during the aggregation process. It is worth noting that although the graph attention network (GAT) can learn attention scores to measure the contribution of neighbors, it still treats each feature channel equally. Then a natural question is how to enable current GNNs with the capability of assigning different smoothness levels to different feature channels. 
% For example, in a social network, user attributes often consist of gender, marital status, interest, location, etc. Two connected users are expected to share similar interest and close location while their gender and marital status could be quite different. 


% Another approach for generating node embeddings falls into graph neural networks, which can capture both structure and feature information simultaneously. \jw{GNN message passing...} However, current GNNs do not specify different smoothness for different feature channels and they may fail to evaluate the contribution from the neighbors fairly. 




% \jw{interpretable?} 

% Motivation: 
% For disassorative graphs, some feature dimension are not smooth (not homophily), we can choose not to aggregate them.


==> tables/node_classification_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[h]
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
                     & \textbf{GCN}   & \textbf{GAT}   & \textbf{SGC}   & \textbf{ARMA}  & \textbf{APPNP} & \textbf{Geom-GCN} & \textbf{Ours-g} & \textbf{Ours-n} & \textbf{Ours-p} & \textbf{\begin{tabular}[c]{@{}l@{}}Improvement \\ over GCN\end{tabular}} \\ \midrule
\textbf{BlogCatalog} & 79.07          & 77.30          & 75.82          & 93.00          & 96.06          & N/A               & \textbf{95.95}  & 95.90           & 96.25           & 17.18                                                                    \\
\textbf{Flickr}      & 66.65          & 61.18          & 45.68          & 90.78          & 91.63          & N/A               & 90.97           & 90.85           & 91.89           & 25.24                                                                    \\
\textbf{Texas}       & 64.00          & 58.46          & 58.81          & 74.19          & 60.76          & 67.57             & 79.84           & 79.92           & 79.81           & 15.92                                                                    \\
\textbf{Wisconsin}   & 61.55          & 60.67          & 59.45          & 73.45          & 63.06          & 64.12             & 81.53           & 82.06           & 82.24           & 20.69                                                                    \\
\textbf{Cornell}     & 58.00          & 59.27          & 58.86          & 67.43          & 65.81          & 60.81             & 80.16           & 79.95           & 79.92           & 22.16                                                                    \\
\textbf{Actor}       & 30.53          & 29.41          & 30.36          & 32.44          & 34.45          & 31.63             & 34.87           & \textbf{34.97}  & \textbf{34.95}  & 4.44                                                                     \\
\textbf{Cora}        & 87.04          & 86.88          & 86.90          & 85.83          & \textbf{85.11} & 85.27             & \textbf{87.04}  & 86.90           & 86.74           & 0.00                                                                     \\
\textbf{Citeseer}    & 76.44          & 76.86          & \textbf{75.38} & 75.91          & 75.95          & \textbf{77.99}    & 76.30           & 76.85           & 76.79           & 0.41                                                                     \\
\textbf{Pubmed}      & \textbf{86.94} & \textbf{86.04} & 81.47          & \textbf{86.62} & 86.65          & 90.05             & 88.12           & 88.15           & 88.12           & 1.21                                                                     \\ \midrule
\textbf{Avg. Rank}   & 5.8            & 6.9            & 7.8            & 5.4            & 5.3            & 4.6               & 2.9             & 2.5             & 2.7             &                                                                          \\ \bottomrule
\end{tabular}
\end{table*}
